Compositional planning in Markov decision processes: Temporal abstraction meets generalized logic composition

In hierarchical planning for Markov decision processes (MDPs), temporal abstraction allows planning with macro-actions that take place at different time scale in form of sequential composition. In this paper, we propose a novel approach to compositional reasoning and hierarchical planning for MDPs under temporal logic constraints. In addition to sequential composition, we introduce a composition of policies based on generalized logic composition: Given sub-policies for sub-tasks and a new task expressed as logic compositions of subtasks, a semi-optimal policy, which is optimal in planning with only sub-policies, can be obtained by simply composing sub-polices. Thus, a synthesis algorithm is developed to compute optimal policies efficiently by planning with primitive actions, policies for sub-tasks, and the compositions of sub-policies, for maximizing the probability of satisfying temporal logic specifications. We demonstrate the correctness and efficiency of the proposed method in stochastic planning examples with a single agent and multiple task specifications.

==> fragment_of_proof_gcd.tex <==

% \begin{align*}
% \pi(s,o_i) =  
%   & \mathsf{softmax}_{d\in \dist{O}} \sum_{o_j \in O} d[j] \sum_{i=1}^n \exp(Q(s, o_i)) \\
%   =&  \frac{1}{\eta}  \frac{\sum_{i=1}^n \exp(\eta x_i^{j})}{\sum_{o_j\in
%         O}\sum_{i=1}^n \exp(\eta x_i^{j}) }
% \end{align*} 

% For each state $s\in S$, let $x_i^j(s)$ be the level of truthfulness for satisfying formula $\varphi_i = \neg \varphi_{\unsafe}\until \sigma_i$ in the Markov chain induced by option $o_j$, the optimal decision rule $d(s): \{O\}\rightarrow [0,1]$ for maximizing the value of GCD $\lambda (x_1,\ldots, x_n\mid \eta)$ is the solution to the following optimization problem:
% \begin{align*}
%   \max_{d \in \dist{O}} \sum_{o_j \in O} d[j] \sum_{i=1}^n \exp(\eta x_i^{j}) 
% \end{align*}
%   Replacing the hardmax with softmax as follows:

%   \begin{align*}
%   & \mathsf{softmax}_{d\in \dist{O}} \sum_{o_j \in O} d[j] \sum_{i=1}^n \exp(\eta x_i^{j}) \\
%   =&  \frac{1}{\eta}  \frac{\sum_{i=1}^n \exp(\eta x_i^{j})}{\sum_{o_j\in
%         O}\sum_{i=1}^n \exp(\eta x_i^{j}) }
%   \end{align*}
% which corresponds to the vector $d$ (the ``soft indmax'') as 
% \begin{equation}
%   d[j] = \frac{\sum_{i=1}^n \exp(\eta x_i^{j})}{\sum_{o_j\in
%       O}\sum_{i=1}^n \exp(\eta x_i^{j}) }, \quad \text{for  }j=1,\ldots, n.
% \end{equation}

% Further, recall that $x_i^j = r_{s}^{o_j}$ is the total accumulated
% reward, \ie, (discounted) probability of satisfying formula
% $\varphi_j$, from state $s$ by following the option $o_j$ in the
% \ac{mdp} $\cal M$ until termination.


% Finally, we define a policy in the semi-\ac{mdp} by
% \begin{equation}
%   \label{eq:comp-policy}
%   \pi(o_j|s) = \frac{\sum_{i=1}^n \exp(\eta r_{s}^{o_j} )}{\sum_{o_j\in
%       O}\sum_{i=1}^n \exp(\eta r_{s}^{o_j}) },\quad \forall s\in S \setminus \unsafe.
% \end{equation}
% \end{proof}


 
% Relating to policy composition, take a Markovian policy
% $\pi:S\rightarrow \dist{A}$, we can interpret $x_i$ as the level of
% truthfulness for satisfying the formula $\varphi_i$ in the Markov
% chain $\mathcal{M} ^\pi$ induced from this policy $\pi$. 

% Recall that for each formula $\varphi_i$, the $i$-th option $o_i= \{\mathcal{I}_i, \pi_i, \beta_i\}$ is defined such that $\pi_i$ is
% the softmax optimal policy for maximizing the probability of
% satisfying $\varphi_i$, and
% $\beta_i(s)= \mathbbm{1}_{ \goal_i\cup \unsafe}(s) $ is the
% termination function. To maximize
% $ \Expect_{M^\pi,s} \left[\lambda(x_1, x_2|\eta)\right]$, given that we
% are only allowed to select options from a given set $o_1,\ldots, o_n$, for a given state $s$ as the initial state,
% the following problem is formulated to compute the decision rule $d$:
% \begin{align*}
%   \max_{d \in \dist{O}} \sum_{o_j \in O} d[j] \sum_{i=1}^n \exp(\eta x_i^{j}) 
% \end{align*}
%   where $x_i^j$ is the level of truthfulness for satisfying formula
%   $\varphi_i$ in the Markov chain induced by option $o_j$.


% \color{blue} 
